Know More, Know Clearer: A Meta-Cognitive Framework for Knowledge Augmentation in Large Language Models

Knowledge augmentation has significantly enhanced the performance of Large Language Models (LLMs) in knowledge-intensive tasks. However, existing methods typically operate on the simplistic premise that model performance equates with internal knowledge, overlooking the knowledge-confidence gaps that lead to overconfident errors or uncertain truths. To bridge this gap, we propose a novel meta-cognitive framework for reliable knowledge augmentation via differentiated intervention and alignment. Our approach leverages internal cognitive signals to partition the knowledge space into mastered, confused, and missing regions, guiding targeted knowledge expansion. Furthermore, we introduce a cognitive consistency mechanism to synchronize subjective certainty with objective accuracy, ensuring calibrated knowledge boundaries. Extensive experiments demonstrate the our framework consistently outperforms strong baselines, validating its rationality in not only enhancing knowledge capabilities but also fostering cognitive behaviors that better distinguish knowns from unknowns. All codes are available at https://github.com/AI9Stars/Know-More-Know-Clearer.

==> figure/Multi_dimensional_cognitive_Evaluationt.tex <==
% 首先需要这些宏定义（放在导言区或figure之前）
\makeatletter
\def\tkz@KiviatGrad[#1](#2){% 
\begingroup
\pgfkeys{/kiviatgrad/.cd,
graduation distance= 0 pt,
prefix ={},
suffix={},
unity=1,
label precision/.store in=\gradlabel@precision,
label precision=1,
zero point/.store in=\tkz@grad@zero,
zero point=0,
}
\pgfqkeys{/kiviatgrad}{#1}% 
\let\tikz@label@distance@tmp\tikz@label@distance
\global\let\tikz@label@distance\tkz@kiv@grad
 \foreach \nv in {0,2,...,\tkz@kiv@lattice}{
 \pgfmathsetmacro{\result}{\tkz@kiv@unity*\nv+ \tkz@grad@zero}
 \protected@edef\tkz@kiv@gd{%
    \tkz@kiv@prefix%
    \pgfmathprintnumber[precision=\gradlabel@precision,fixed]{\result}%
    \tkz@kiv@suffix} 
    \path[/kiviatgrad/.cd,#1] (0:0)--(360/\tkz@kiv@radial*#2:\nv*\tkz@kiv@gap)
       node[label={[label distance=0.01em](360/\tkz@kiv@radial*#2):\tiny\tkz@kiv@gd}] {};
      }
 \let\tikz@label@distance\tikz@label@distance@tmp  
\endgroup
}%

\def\tkz@KiviatLine[#1](#2,#3){% 
\begingroup
\pgfkeys{/kiviatline/.cd,
fill= {},
opacity=.15,
zero point/.store in=\tkz@line@zero,
zero point=0
}
\pgfqkeys{/kiviatline}{#1}%
\ifx\tkzutil@empty\tkz@kivl@fill \else 
\path[fill=\tkz@kivl@fill,opacity=\tkz@kivl@opacity] (360/\tkz@kiv@radial*0:{(#2+\tkz@line@zero)*\tkz@kiv@gap*\tkz@kiv@step})   
\foreach \v [count=\rang from 1] in {#3}{%  
 -- (360/\tkz@kiv@radial*\rang:{(\v+\tkz@line@zero)*\tkz@kiv@gap*\tkz@kiv@step}) } -- (360/\tkz@kiv@radial*0:{(#2+\tkz@line@zero)*\tkz@kiv@gap*\tkz@kiv@step});
 \fi
\draw[#1,opacity=1,overlay] (0:{(#2+\tkz@line@zero)*\tkz@kiv@gap}) plot coordinates {(360/\tkz@kiv@radial*0:{(#2+\tkz@line@zero)*\tkz@kiv@gap*\tkz@kiv@step})}  
\foreach \v [count=\rang from 1] in {#3}{%  
 -- (360/\tkz@kiv@radial*\rang:{(\v+\tkz@line@zero)*\tkz@kiv@gap*\tkz@kiv@step}) plot coordinates {(360/\tkz@kiv@radial*\rang:{(\v+\tkz@line@zero)*\tkz@kiv@gap*\tkz@kiv@step})}} -- (360/\tkz@kiv@radial*0:{(#2+\tkz@line@zero)*\tkz@kiv@gap*\tkz@kiv@step});   
\endgroup
}%  

\def\tkz@KiviatDiagram[#1]#2{% 
\pgfkeys{/kiviat/.cd,
gap          = .5,
lattice      = 10,
space        = .5,
step         = 1, 
label space  = 1.5
}
\pgfqkeys{/kiviat}{#1}%
\begingroup
\foreach \x [count=\rang from 1] in {#2}{%
\global\let\tkz@kiv@radial\rang}% 
\foreach \x [count=\rang from 0] in {#2}{%
   \draw[/kiviatfile/radial style2]
 (0,0)--(360/\tkz@kiv@radial*\rang:\tkz@kiv@lattice*\tkz@kiv@gap+\tkz@kiv@sp);
   \path
(0,0)--(360/\tkz@kiv@radial*\rang:\tkz@kiv@lattice*\tkz@kiv@gap+\tkz@kiv@space) node[/kiviat/label style] {\x}; 

\foreach \y in {1,...,\tkz@kiv@lattice}{
   \draw[/kiviat/lattice style]%
     (360/\tkz@kiv@radial*\rang:\y*\tkz@kiv@gap)--%
        (360/\tkz@kiv@radial*\rang+360/\tkz@kiv@radial:\y*\tkz@kiv@gap);
}
}
\endgroup
}

% Legend环境定义
\newenvironment{customlegend}[2][]{%
    \begingroup
    \pgfplots@init@cleared@structures
    \pgfplotsset{#1}%
    \begin{scope}[shift={#2}]
}{%
    \pgfplots@createlegend
    \end{scope}
    \endgroup
}%

\def\addlegendimage{\pgfplots@addlegendimage}
\makeatother

% 颜色定义
\definecolor{c0}{HTML}{ffffff}
% \definecolor{c1}{HTML}{CE93D8}
% \definecolor{c2}{HTML}{ff8c1a}
% \definecolor{c5}{HTML}{00aeef}
% \definecolor{c9}{RGB}{149, 188, 143}
% \definecolor{c10}{RGB}{132, 211, 222}
% \definecolor{c11}{RGB}{235, 72, 63}

\definecolor{c1}{HTML}{6BAED6}
\definecolor{c2}{HTML}{A93226}
\definecolor{c5}{HTML}{2E8B57}
\definecolor{c9}{HTML}{3A6EA5}
\definecolor{c10}{HTML}{E69F00}
\definecolor{c11}{HTML}{1F3A5F}

% 柱状图颜色
\definecolor{upink}{HTML}{fcd4d4}
\definecolor{ucyan}{HTML}{e3eeff}
\definecolor{uedgecyan}{HTML}{6d97e0}
\definecolor{uedgepink}{HTML}{cc0000}

% 然后是图形部分
\begin{figure}[t]
    \centering
    \begin{tikzpicture}[
      label distance=13em,
      plot1/.style={semithick, draw=c1, fill=c0, mark=triangle*, mark options={color=c1, mark size=3pt}, opacity=.15},
      plot2/.style={semithick, draw=c2, fill=c0, mark=triangle*, mark options={color=c2, mark size=3pt}, opacity=.15},
      plot5/.style={semithick, draw=c5, fill=c0, mark=triangle*, mark options={color=c5, mark size=3pt}, opacity=.15},
      plot9/.style={semithick, draw=c9, fill=c0, mark=triangle*, mark options={color=c9, mark size=3pt}, opacity=.15},
      plot10/.style={semithick, draw=c10, fill=c0, mark=triangle*, mark options={color=c10, mark size=3pt}, opacity=.15},
      plot11/.style={semithick, draw=c11, fill=c0, mark=triangle*, mark options={color=c11, mark size=3pt}, opacity=.15},
    ]
    
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  
    % 左侧: 柱状图 (占总宽度的40%)
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \begin{scope}[scale=0.88]  % 缩小到85%
    \begin{axis}[
      at={(0,0)},
      ymajorgrids,
      grid style=dashed,
      ybar=1pt,
      enlarge x limits=0.05,
      xtick align=inside,
      width=0.3\textwidth,        % 缩小到0.2倍文本宽度
      height=0.3\textwidth,      % 相应调整高度
      bar width=0.8em,            % 缩小柱宽
      ylabel={\scriptsize Answerable Accuracy (\%)},
      ylabel style={yshift=-1.5em, font=\scriptsize}, 
      nodes near coords,
      nodes near coords align={vertical},
      nodes near coords style={
  font=\tiny, 
  /pgf/number format/fixed, 
  /pgf/number format/fixed zerofill, 
  /pgf/number format/precision=2  % ← 这里要加 /
},
      xmax=6.5,
      xmin=0.5,
      xtick=data,
      ymin=0,
      ymax=60,
      ytick={0,20,40,60},         % 减少刻度数量
      yticklabels={0,20,40,60},
      xticklabels={Vanilla LLM , Know What, CRew-DPO, BARREL, GRPO, Ours},  % 缩短标签
      xtick style={draw=none},
      yticklabel pos=left,
      yticklabel style={/pgf/number format/fixed, font=\tiny},
      xticklabel style={rotate=45, anchor=east, font=\tiny},
      axis on top=false,
    ]
      \addplot[fill=ucyan, draw=uedgecyan, area legend] coordinates { 
        (1,31.66) (2,29.10) (3,19.26) (4,27.77) (5,46.56) (6,49.21)
      };
    \end{axis}
\end{scope}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  
    % 右侧: 雷达图 (占总宽度的60%)
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \begin{scope}[
      shift={(5.2cm, 1.5cm)},     % 调整位置使其紧邻柱状图
      scale=0.16,                 % 缩小雷达图
    ]
    
      % 定义宏
      \def\KivStep{0.1}
      \pgfmathsetmacro\Unity{1/\KivStep}
      \def\zeroshift{0}

      % 绘制雷达图
      \tkzKiviatDiagram[
        radial style2/.style={-},
        rotate=90, 
        lattice style/.style={black!30},
        label style/.style={font=\tiny},    % ← 添加这一行，设置标签字体
        step=\KivStep,
        gap=1,
        lattice=9,
      ]{AR, KEI, CBS, CAE, NPV}

      % 数据线
      \tkzKiviatLine[plot5](79.74, 57.60, 66.88, 60.43, 41.05)
      \tkzKiviatLine[plot2](71.64, 2.05, 3.99, 31.49, 30.68)
      \tkzKiviatLine[plot1](72.13, 20.15, 31.51, 39.21, 31.30)
      \tkzKiviatLine[plot9](70.44, 24.78, 36.66, 40.61, 30.98)
      \tkzKiviatLine[plot10](89.84, 21.18, 34.28, 43.66, 34.63)
      \tkzKiviatLine[plot11](87.27, 63.37, 73.43, 68.18, 48.80)
      
      \tkzKiviatGrad[unity=\Unity, label precision=0, zero point=\zeroshift](0)
      
      % 雷达图图例 (放在下方)
      \begin{customlegend}[
        legend columns=2,         % 改为3列以节省空间
        legend style={draw=none, column sep=0.5ex, font=\tiny},
        legend entries={Vanilla LLM , Know What, CRew-DPO, BARREL, GRPO, Ours}
      ]{(-30em,-45em)}            % 调整图例位置
        \addlegendimage{c5, fill=c5, mark=triangle*, sharp plot}
        \addlegendimage{c2, fill=c2, mark=triangle*, sharp plot}
        \addlegendimage{c1, fill=c1, mark=triangle*, sharp plot}
        \addlegendimage{c9, fill=c9, mark=triangle*, sharp plot}
        \addlegendimage{c10, fill=c10, mark=triangle*, sharp plot}
        \addlegendimage{c11, fill=c11, mark=triangle*, sharp plot}
      \end{customlegend}
      
    \end{scope}

    \end{tikzpicture}
    \caption{Performance Comparison across Different Metrics on the Qwen2.5-7B-Instruct. Left: Answerable accuracy. Right: Multi-dimensional evaluation on AR, KEI, CBS, CAE, and NPV metrics.}
    \label{fig:multi-dimensional}
\end{figure}
